KROME - a package to embed chemistry in astrophysical simulations

Chemistry plays a key role in many astrophysical situations regulating the cooling and the thermal properties of the gas, which are relevant during gravitational collapse, the evolution of disks and the fragmentation process. In order to simplify the usage of chemical networks in large numerical simulations, we present the chemistry package KROME, consisting of a Python pre-processor which generates a subroutine for the solution of chemical networks which can be embedded in any numerical code. For the solution of the rate equations, we make use of the high-order solver DLSODES, which was shown to be both accurate and efficient for sparse networks, which are typical in astrophysical applications. KROME also provides a large set of physical processes connected to chemistry, including photochemistry, cooling, heating, dust treatment, and reverse kinetics. The package presented here already contains a network for primordial chemistry, a small metal network appropriate for the modelling of low metallicities environments, a detailed network for the modelling of molecular clouds, a network for planetary atmospheres, as well as a framework for the modelling of the dust grain population. In this paper, we present an extended test suite ranging from one-zone and 1D-models to first applications including cosmological simulations with ENZO and RAMSES and 3D collapse simulations with the FLASH code. The package presented here is publicly available at http://kromepackage.org/ and https://bitbucket.org/krome/krome_stable

==> basic_usage.tex <==
\section{Basic usage and options}\label{sect:basic_usage}
\krome acts as a pre-processor to provide the necessary \fortran files that allows to compute the chemical evolution in the framework code. The simplest way to create these files is to type in a standard Unix shell\footnote{Note that \krome has been developed under Ubuntu Linux and is never been tested with accuracy on MS Windows\trader systems, even if in principle it suffices that a \python interpreter and the \textsc{LAPACK} libraries when metal cooling is present. For this reason \krome has been successfully tested on OSX systems.} when the current path is the main \krome folder
\begin{verbatim}
> ./krome -n network
\end{verbatim}
where \verb+network+ is a CSV file of the chemical networks where each line contains the information on each reaction that belongs to the network. For example, the electron attachment on hydrogen ($\mH+\me^-\to\mH^-+\gamma$) is
\begin{verbatim}
9, H, E, , H-, g, , , 10, 1e8, 6.77d-15*Te**0.878d0
\end{verbatim}
with $T_e$ the electronic temperature in eV. The strings has the following default template
\begin{verbatim}
index, R1, R2, R3, P1, P2, P3, P4, Tmin, Tmax, rate
\end{verbatim}
where \verb+R1+ to \verb+R3+ are the three reactants, \verb+P1+ to \verb+R4+ the four products, \verb+Tmin+ and \verb+Tmax+ the temperature limits in K, and \verb+rate+ is the rate coefficients in the \fortran format\footnote{The double precision is not mandatory, but in the code the non-double precision expression will be replaced with the correct one, since \krome works in the double precision format. Moreover, some compilers may replace non-double numbers.} 
but in principle can be modified according to different formats within the reaction file thanks to customary strings (see Appendix \ref{appx:file_format}).
Note also that the reaction file allows in-line comments (line starting with \verb+#+), multi-line comments (using the classic \textsc{C++} \verb+\*+ and \verb+*/+ tokens), blank lines and variable initializations for variable-depending rates, or rates that needs more complex expressions, e.g.
\begin{verbatim}
	@var:a = 1d3/T
\end{verbatim}
to define the variable \verb+a+ that can be employed in all the \fortran rate expressions that are present in the reaction file. Note that in the present release \krome follows the order of the variables found in the file and always uses double precision (\verb+real*8+).

To modify the behaviour of the pre-processing there are several options that can be appended to the call to the command \verb+krome+. We briefly describe them here, but refer to the manual for further information and examples or directly ask to the authors.
\begin{itemize}
	\item \verb+-iRHS+ this option uses an implicit coding for the RHS of Eq.(\ref{eqn:ODEs}) instead the explicit one, which is the default. This issue is discussed in detail in Sect.\ref{sect:implicitODE} above. It is very useful for large systems ($\gtrsim500$ reactions) to save time during the compilation. Note that with this options the calculation could be slower.

	\item \verb+-forceMF=21+ forces the MF value of the solver to the value 21 which means that the Jacobian and the sparsity matrix is not calculated by the solver but is explicitly determined by \krome and passed to the solver at run-time (see Sect.\ref{sect:solver} and \dlsodess/\textsc{DVODE} manuals).

	\item \verb+-forceMF=222+ forces the MF value of the solver to 222 which means that the Jacobian and the sparsity matrix are calculated by the solver at runtime (see Sect.\ref{sect:solver} and the solver manuals).

	\item \verb+-test=TEST+ The \krome package has a set of tests to help the user with the implementation of the different options that this code provides. These tests are discussed in Sect.\ref{sect:test_suite} in detail, while here we only make a list of the possible strings for \verb+TEST+:  \verb+atmosphere+ is a simple layered planet atmosphere with chemistry coupled with diffusion, \verb+cloud+  is the one-zone model of \citet{Wakelam2008} without PAHs, \verb+collapse+ is a standard gravitational collapse \citep{Omukai2000}, \verb+collapseUV+ is the same model with molecular hydrogen photodissociation enabled, \verb+collapseZ+ with metals, \verb+compact+ is an example to show the compact version of the modules of \krome that is useful to embed the package in framework codes without many \fortran files, \verb+dust+ is a warming medium with graphite and silicate dust, including growth and sputtering, \verb+lotkav+ is a Lotka-Volterra ODE system, \verb+map+ shows the evolution of the ISM changing two parameters, i.e. density and UV flux intensity, \verb+reverse+ is a nitric oxide (NO) mechanism with reverse kinetics, \verb+shock1D+ is a one-dimensional shock with a primordial chemical network, \verb+shock1Dcool+ is the same model but with cooling, \verb+shock1Dphoto+ has the reactions of photoionization and the relative heating, \verb+slowmanifold+ tests the slow-manifold theory with a simple network, and \verb+wrapC+ shows how to call \krome from a C program.

%"ATOMIC","H2","HD","Z","DH","DUST","H2GP98","COMPTON","CIE",
%"CI","CII","SiI","SiII","OI","OII","FeI","FeII","CONT","CHEM"
\item \verb+-cooling=COOLING+ This option allows to compute the cooling at run-time. \krome is a package that is mainly developed for astrophysical applications, and in particular the cooling is developed for primordial and metal-enriched environments. For this reason we provide several kind of cooling that can be included replacing the token \verb+COOLING+ with a comma-separated list that includes the following options (see Sect.\ref{sect:cooling}): \verb+ATOMIC+ for \citet{Cen1992} cooling, \verb+H2+ for molecular hydrogen with the \citet{Glover2008} recipe and \verb+H2GP+ for the \citet{Galli1998} one, \verb+HD+ using \citet{Lipovka2005} model, \verb+Z+ for metals using \citet{Maio2007} extended with \citet{Grassi2012}, and, \verb+COMPTON+ is the Compton cooling, \verb+CIE+ is the collisional induced cooling, \verb+CONT+ the continuum from the gas, \verb+CHEM+ is due to the reactions following \citet{Omukai2000}, and finally \verb+CI+ and its analogous are helpful to enabled single metal cooling contributions. An example is the \verb+-cooling=CI,OII,H2,HD+ option, which enable C and O$^+$ line cooling, molecular hydrogen and HD cooling. 


\item \verb+-heating=HEATING+ The heating option is analogous to the cooling one. It allows to choose the desired heating functions for the modelled environment. The options follows the scheme in Sect.\ref{sect:heating} where \verb+COMPRESS+ is the compressional heating, \verb+CHEM+ is the heating from the formation of molecular hydrogen and other processes, \verb+PHOTO+ is the photoionization heating that is enabled for the photoionization reactions included in the chemical network (see the relative option), and \verb+DH+ is the enthalpic heating. An example is given in the test \verb+shock1Dphoto+ that represents a monodimensional shock with a primordial chemical network that includes cooling and photoionization heating for atoms and molecules.

	\item \verb+-useN+ \krome can build an interface that works both with number densities, and mass fractions (if the total density is provided). This option allows to use number densities (cm$^{-3}$) instead of the default mass fractions (dimensionless). It is worth noting that the \krome interface in the framework program changes from
\begin{verbatim}
call krome(x(:), rho, Tgas, dt)
\end{verbatim}
to 
\begin{verbatim}
call krome(x(:), Tgas, dt)
\end{verbatim}
where \verb+x(:)+ represents the array of the species (mass fractions in the first case, number densities in the second), \verb+rho+ is the total gas density (g cm$^{-3}$), and \verb+dt+ is the integration time-step in seconds. When this option is not enabled \krome employs the following conversion at run-time since the solver requires number densities:
\begin{equation}
	n_i = \frac{\rho\,x_i}{m_i}\,,
\end{equation}
where $n_i$ is the number density of the \ith species (cm$^{-3}$), $\rho$ is the total density of the gas (g cm$^{-3}$), $x_i$
the mass fraction (dimensionless), and $m_i$ the mass of the species (g).



	\item \verb+-useH2opacity+ includes density dependent H$_2$ opacity for H$_2$ and collisional induced cooling following \citet{Ripamonti2004}.

	\item \verb+-gamma=OPTION+ provides an expression for the adiabatic index $\gamma$ (e.g. \verb+gamma="5d0/3d0"+), or using \verb+gamma=FULL+ \krome computes a chmistry-dependent $\gamma$ as in Eq.(\ref{eq:adiabatic}). 

	\item \verb+-maxord=N+ forces the maximum order of integration. The default (and the largest allowed) value is 5.

	\item \verb+-ATOL=N+ sets the absolute tolerance of the solver to the value N. The default value is $10^{-40}$ which ensures the stability for most of the chemical networks, even if a higher values are suggested to reduce the integration time in CPU-demanding models (see Sect.\ref{sect:solver} and the solver manuals). Note that individual ATOLs can be indicated by using the \verb+-customATOL=FILENAME+ option (see the relative option).

	\item \verb+-RTOL=N+ sets the relative tolerance of the solver to the value N. The default value is $10^{-6}$, and the same discussion made for ATOL can be applied here.


	\item \verb+-customATOL=FILENAME+ provides a user-defined space-separated file with the list of the ATOL for the different species. The user can indicate the explicit name of the species and the value (e.g. \verb#H+ 1d-2#), with a species per line. The species not included in the file have ATOL equal to the default value (\kromes's default or indicated by the user via \verb+-ATOL+ option). Comments in the file are allowed (lines starting with \verb+#+).

	\item \verb+-customRTOL=FILENAME+ Analogous option employed for ATOL above.

\item \verb+-usePhIoniz+ It must be activated when the network presents reactions that include photons in the reactants and for which a rate cross section is available. The behaviour of these reactions follows the scheme presented in Sect.\ref{sect:phioniz},  and the user must provide the reaction cross section as a function of the energy, or, in case of atoms and their ions, use the internal generated cross sections from \citet{Verner1996}. The temperature limits of the reaction in this case are the energy limits, and the rates must be indicated by prepending the statement \verb+krome_kph_auto=+ in the rate slot. An example is provided by the network file \verb+networks/react_primordial_photo+ used in the test \verb+shock1Dphoto+.

\item \verb+-useEquilibrium+ In most of the photoionization processes the accuracy of the solver is too low and it can generate an oscillating behaviour that may result in a solver slow down that can freeze the system. In this case we employ a criterion to determine if the system has reached an oscillating equilibrium and can be safely stopped:
\begin{equation}
 \frac{\left|n_i(t+\Delta t)-n_i(t)\right|}{n_i(t+\Delta t)}<10^{-6}\,\, \forall i \in species\,.
\end{equation}
In the above equation $n_i(t+\Delta t)$ and $n_i(t)$ are the numerical abundances of the \ith species after and before the call to the solver inside an iteration time-step (see Sect.\ref{sect:solver}). \emph{This option should be used with extremely caution}.


\item \verb+-dust=N,TYPE1,TYPE2,...+ the dust is included following the model shown in Sect.\ref{sect:dust}, where the dust is subdivided into \verb+N+ bins times the types of dust employed. The dust can be carbon-based (graphite) or silicon-based (silicates) and the option \verb+TYPE+ allows to determine what grains are used. An example is \verb+-dust=10,C,Si+ that creates 10 bins of dust of graphite and 10 bins of silicates. In this public release of \krome we include the data only for this two types of dust, but in principle the user can add his/her own dust models. The test for the dust is provided in Sect.\ref{sect:test_dust}, that represents a one-zone model with two dust types that evolve into a warming medium. Finally, this option requires a mandatory call to the subroutine \verb+krome_init_dust+ which initialises the dust following the MRN distribution of Sect.\ref{sect:dust} ($\alpha=-3.5$).

\item \verb+-dustOptions=OPTIONS+ activates the options related to the dust processes. \verb+OPTIONS+ should be one of following: \verb+H2+ for H$_2$ formation on dust following  \citet{Cazaux2009}, \verb+GROWTH+ as in Sect.\ref{sect:growth}, and \verb+SPUTTER+ for thermal sputtering as described in Sect.\ref{sect:sputter} above. Example: \verb+-dustOptions=H2,SPUTTER+ to include molecular hydrogen grain catalysis and thermal sputtering.

\item \verb+-compact+ allows a compact form for the generated \fortran files, while (by default) \krome generates a file for each module, where each module represents a group of related physical processes. This option is intended to have a more compact list of files to be included in the Makefile of the framework code. It generates a \verb+krome_all.f90+ file and \verb+krome_user_commons.f90+ to allow an easier modification of this module only. However, with this flag the file of the solvers are not embedded in the compact file and must be included in the Makefile as for the default multi-files mode.

\item \verb+-useDvodeF90+ prepares the interface for the \textsc{DVODE} in its \fortran 90 version\footnote{\arl{http://www.radford.edu/~thompson/vodef90web/}}. Note that not all the \krome options are available when this flag is active.  

\item \verb+-useTabs+ with this option \krome uses discrete values for the rate coefficients and employ them to retrieve the approximated rate values by linear interpolation. This option should be used when the rates have complex \fortran expression (logarithms, exponentials, and similar functions), while it causes an overload when rates are composed by constant values or simple expressions.

\item \verb+-report+ tracks some variables that play a key role for finding problems during the solver integration. When it is enabled the \fortran code produces at run-time two files (\verb+KROME_ERROR_REPORT+ and \verb+KROME_ODE_REPORT+) that contain the status of the system, and \fortran file on unit 98 (namely \verb+fort.98+) that dump the abundances of the species at each call of the $FEX$ routine (see Sect.\ref{sect:code_structure}). Note that this option is only intended for debug purposes, since it reduce the efficiency of the code.

\item \verb+-checkConserv+ checks the total mass conservation at run-time and stop the execution when the following criterion is not satisfied:
\begin{equation}\label{eqn:conserv}
	\left|1-\frac{\sum n_i(t)\,m_i}{\sum n_i(t+\Delta t)\,m_i}\right|<10^{-3}\,,
\end{equation}
where $n_i(t)$ and $n_i(t+\Delta t)$ are the number densities of the \ith species evaluated before and after the solver integration, respectively. The quantity on the LHS of Eq.(\ref{eqn:conserv}) is equal to zero when the total mass is perfectly conserved.

\item \verb+-useFileIdx+ without this option \krome use its own reaction index, otherwise it uses the indexes provided in the reaction file by the user. This option is useful when the rates depends on previously calculated rate values (e.g. $k(11) = 0.5\,[k(10)+k(2)]$).
 

	\item \verb+-forceRWORK=N+ forces the size of RWORK to the value N. This helps when \krome and/or the solver have problems in determining the size of the real array employed to communicate between the solver and the routine that calls the solver (see Sect.\ref{sect:solver} and the DLSODES/DVODE manuals).

	\item \verb+-skipDup+ skip duplicate reactions. Note that if the reactions with the same reactants and products have different temperature range \krome can't distinguish them. Use with caution.

	\item \verb+-Tlimit=opLow,opHigh+ determines the binary operators used to determine the validity of the rate coefficient respect to the lower and the upper temperature limits. Default operators are $T\ge T_\mathrm{min}$ (GE) and  $T< T_\mathrm{max}$ (LT). Operators must be one of the following GT (for $>$), GE ($\ge$), LT ($<$), and LE ($\le$). Example \verb+-Tlimit=GT,LE+ provides $T> T_\mathrm{min}$ and  $T\le T_\mathrm{max}$. Note that operators for individual reactions can be indicated in the reaction file.

	\item \verb+-noTlimits+ removes all the temperature limits and the \verb+if+ statements in the \fortran files.

	\item \verb+-reverse+ creates inverse reactions using NASA polynomials as discussed in Sect.\ref{sect:reverse}.

	\item \verb+-useCustomCoe=FUNCTION+ forces to employ a custom function for the rate coefficient instead of using the \kromes-generated one. The function must be provided by defining it in the \verb+krome_user_commons.f90+ file.

	\item \verb+-useODEConstant=EXPRESSION+ postpones a \fortran expression to all the ODEs in the $FEX$ routine. \verb+EXPRESSION+ must be a valid \fortran expression starting with an operator (i.e. \verb#+, -, *, /#).

	\item \verb+-skipODEthermo+ enabling this option \krome will not include the $\dd T/\dd t$ expression in the $FEX$ routine even if cooling and/or heating options are enabled. It is intended for debug purposes.

	\item \verb+-usePlainIsotopes+ \krome can handle nuclear networks that includes isotopes. The default syntax for isotopes is $[N]$A, where $N$ is the mass number and A is the name of the element (e.g. $[14]$C), but when this flag is present \krome searches for the $N$A form (e.g. $14$C). 

	\item \verb+-project=PROJECTNAME+ with this option \krome builds the file in the \verb+/build_PROJECTNAME+ directory and produces a .kpj file that stores the command line employed.

	\item \verb+-clean+ cleans all the files the \verb+/build+ folder before building the new project.

	\item \verb+-pedantic+ copies the pedantic Makefile with all the most important debug options instead of the default Makefile that uses aggressive optimization options.

	\item \verb+-ramses+, \verb+-flash+, \verb+-enzo+ provide the patch for \ramsess, \flashs, and \enzo in the \verb+/build+ folder. More details in the online documentation.

	\item \verb+-C+ provides a \verb+krome.h+ file containing all the necessary includes for framework codes written in C language. The test \verb+-test=wrapC+ shows an example on how to call \krome from a C program.

	\item \verb+-customODE=FILENAME+ provides the name of a file containing custom ODE functions written in \fortran language. More details in the Sect.\ref{sect:test_lotkav} where this option is employed to implement a Lotka-Volterra model. 

\end{itemize}


==> computational_remarks.tex <==
\section{Computational remarks}\label{sec:computational}


==> cooling_plot.tex <==
\subsection{Cooling plot}\label{sect:test_cooling_plot}
\krome has several cooling options that have been described in Sect.\ref{sect:cooling}. The user can plot the cooling functions for different values of temperature by using an utility command \verb+plot_cool(n)+, where $n$ is an array that contains the abundances of the species. This command evaluate the cooling functions in the range $10<T<10^8$ K and save them to a file.

The command line to generate the test is
\begin{verbatim}
 > ./krome -test=cooling
\end{verbatim}
which is a short-cut for 
\begin{verbatim}
 > ./krome network/react_primordial -cooling=ALL 
   -useN
\end{verbatim}
where the reaction network determines only the species used and the reactions that are employed to evaluate the cooling from enthalpy of formation. The option \verb+-cooling=ALL+ turns on all the coolings together, namely CEN, H2, H2GP98, HD, Z, and DH.

In this test we show the cooling by \citet{Cen1993} (CEN93), the molecular hydrogen cooling both by \citet{Galli1998} (H$_2$GP98) and \citet{Glover2008} (H$_2$GA08), HD of \citet{Lipovka2005} (HD), metal cooling (Z), and cooling from the enthalpy of formation ($\Delta$H).
The abundances of the species to obtain this plot are arbitrarily chosen and are listed in Tab.\ref{tab:cooling_init}.
We note here that this test is substantially different from the results reported in Fig. \ref{fig:katz96} where the species abudnances are evolved based on equilibrium assumptions instead to be constant for any temperature as in this case.

\begin{table}
	\caption{Number densities for the cooling test, where $a(b)=a\times10^b$. All the abundances are in units of $10^3$ cm$^{-3}$ for the cooling test (Sect.\ref{sect:test_cooling_plot}), while they represent mass fractions for the shock test (Sect.\ref{sect:test_shock_chem}). \label{tab:cooling_init}}
	\centering
	\begin{tabular}{l|l|l|l}
		\hline
		Species & Abundance & Species & Abundance\\	
		\hline
		H & 0.9225 		& H$_2^+$ & 1.0(-20)\\
		e$^-$ & 1.0(-4) 	& HD & 1.0(-8)\\
		H$^+$ & 1.0(-4) 	& H$^-$ & 1.0(-20)\\
		D & 1.0(-20)	 	& He$^{++}$ & 1.0(-20)\\
		D$^+$ & 1.0(-20) 	& C$^+$ & 1.0(-6)\\
		He & 0.0972 		& Si$^+$ & 1.0(-7)\\
		He$+$ & 1.0(-20) 	& O & 1.0(-4)\\
		H$_2$ & 1.0(-5)		& Fe$^+$ & 1.0(-8)\\
		\hline
	\end{tabular}
\end{table}

\begin{figure}
 \includegraphics[width=.45\textwidth]{figs/test_cooling/test_cooling.eps}
 \caption{Cooling functions at different gas temperature $T_\mathrm{gas}$. Labels are CEN93 for \citet{Cen1993}, H$_2$GP98 and H$_2$GA08 for the molecular hydrogen cooling by \citet{Galli1998} and \citet{Glover2008} respectively, HD for \citet{Lipovka2005}, Z for metal cooling (carbon, silicon, oxygen, and iron), and $\Delta$H for enthalpy of formation cooling. This plot refers to the abundances listed in Tab.\ref{tab:cooling_init}. \label{fig:test_cooling}}
\end{figure}


==> lotkav_test.tex <==
%---------------------------------------------------------------------------
\subsection{Extra ODEs}\label{sect:test_lotkav}
\krome has the capability of handling extra ODE equations to be included in the system of Eq.(\ref{eqn:ODEs2}). These extra equations can be included simply indicating their \fortran expression in a user-defined file.
To provide an example we develop a simple predator-prey Lotka-Volterra model in wich the two populations change according to 
\begin{eqnarray}\label{eqn:LV}
	\frac{\dd x}{\dd t} &=& x\,(a-by)\nonumber\\
	\frac{\dd y}{\dd t} &=& y\,(cx-d)\,\,
\end{eqnarray}
where $x$ and $y$ are the prey and the predator populations respectively, while $a$, $b$, $c$, and $d$ are the paramters that describe the interaction between the two species.
In our case trough the ODE file we provide Eqs.(\ref{eqn:LV}) and the parameters values, namely $a=1$, $b=0.2$, $c=0.04$, and $d=0.5$, which lead an oscillating system as shown in Fig.\ref{fig:LV} that represents the evolution with inital conditions $x_0=5$ and $y_0=2$. The results found match the expected ones.

The command line to generate the test is
\begin{verbatim}
 > ./krome -test=lotkav
\end{verbatim}
which is a short-cut for 
\begin{verbatim}
 > ./krome -n network/dummy 
    -useN
    -customODE=tests/lotkav/lotkav
\end{verbatim}
where the flag \verb+customODE+ allows to suggest a file containing the ODEs, and \verb+network/dummy+ is a dummy network to allow using \krome for non-chemical problems.




\begin{figure}
 	\includegraphics[width=0.48\textwidth]{figs/test_lotkav/lotkav.eps}
         \caption{Time evolution of the prey (solid) and the predator (dahsed) population by using the Lotka-Volterra model of Eqs.(\ref{eqn:LV}).}
 \label{fig:LV}
\end{figure}


==> map_test.tex <==
\subsection{Map}\label{sec:map}
The following test represents a series of one-zone models varying the impinging radiation via the photon flux in the range $10^{-3}<J_{21}<10$ (dimensionless) and the gas density as $10^{-25}<\rho<10^{-21}$ g~cm$^{-3}$. The initial conditions (mass fractions) are $x_\mH=0.9220$, $x_{\me^-}=10^{-4}$, $x_{\mH^+}=10^{-4}$, $x_\mathrm{He}=0.0972$, $x_\mathrm{H_2}=10^{-5}$, and $x_\mathrm{HD}=10^{-8}$,  with an initial temperature of $T=10^4$ K. The physical processes included are H$_2$, HD, atomic cooling, and chemical and photochemical heating. We follow the evolution of the gas until the free-fall time, see \eqnrefs{eqn:ff_time}. The output temperature is plotted in Fig.\ref{fig:mapTgas} together with the mass fraction of H$_2$: as expected the gas is colder where the cooling from molecular hydrogen is more efficient. The cooling efficiency is controlled by the density, which increases the coolant collisions, and by the background radiation, that heats the gas and dissociates the molecular hydrogen. In the upper left region (low density, high flux) the effects of the heating is maximized, as well as in the lower right one (high density, low flux), where the cooling is more efficient and the radiative heating is comparably negligible. In the lower left and in the upper right areas the two effects are nearly comparable. The Fig.\ref{fig:mapTgas} also reports the contour lines for the final mass fractions of H$_2$ which is more abundant in the high density / low flux region.

The command line to generate the test is
\begin{verbatim}
 > ./krome -test=map
\end{verbatim}
which is a short-cut for 
\begin{verbatim}
 > ./krome -n network/react_primordial_UV 
   -cooling=ATOMIC,HD,H2
   -heating=PHOTO
   -usePhIoniz
\end{verbatim}
where \verb+ATOMIC+, \verb+H2+, and \verb+HD+ are the corresponding cooling options, while \verb+PHOTO+ represents the heating from the photoionisation. The option \verb+usePhIoniz+ suggests the use of photochemistry to \kromes.


\begin{figure}
	\includegraphics[width=0.45\textwidth]{figs/test_map/mapTgas.eps}
        \caption{Final gas temperature for models with different $J_{21}$ and density values. We also report the contour lines for the final mass fraction of H$_2$.}\label{fig:mapTgas}
\end{figure}
  

 



==> reverse_test.tex <==
%---------------------------------------------------------------------------
\subsection{Reverse kinetics}\label{sect:test_reverse}
To test the method to derive inverse reactions outlined in Sect.\ref{sect:reverse} we present here a simple problem based on the Zel'dovich thermal nitric oxide (NO) mechanism as discussed in \citet{Ashraf2009}.
This model is based on two forward reactions and the corresponding reverse reactions (see Tab.\ref{tab:NO}) with the rate coefficients taken from \citet{Baulch1994}.



To prove the robusteness of the method employed in \kromes, the reverse rate coefficients ($k_r$) computed with the package are reported in Fig.\ref{fig:reverse_kr} and compared to the experimental and theoretical data from \citet{Baulch1994}, which are fairly matched. We also report the evolution of the abundances of the five species based on the initial condtions of \citet{Ashraf2009}, i.e. $n=10^{-3}$ mol for all the species, volume $V=10^3$ cm$^3$, and $T=4000$ K. The full dynamics of the system is depicted in Fig.\ref{fig:reverse_evol} which matches the analogue Fig.1 of \citet{Ashraf2009}.


The command line to generate the test is
\begin{verbatim}
 > ./krome -test=reverse
\end{verbatim}
which is a short-cut for 
\begin{verbatim}
 > ./krome network/react_NO 
    -useN 
    -reverse
\end{verbatim}
where the flag \verb+reverse+ activates the calculation of the reverse kinetics.

\begin{table}
	\begin{center}
		\caption{Chemical network for the Zel'dovich nitric oxide mechanism, that consists in two forward reactions and two reverse, which are computed with the methodology described within the text.} \label{tab:NO}
		\begin{tabular}{cccl}
		  \hline
		  \multicolumn{3}{l}{Reaction} & $k_{f}$ (cm$^{-3}$ s$^{-1}$) \\
		  \hline
		 N$_2$ + O & ${\overset{k_{f}}{\rightleftharpoons}}$ & NO + N & $3\times10^{-10}\exp(-38300/T)$\\
		 O$_2$ + N & ${\overset{k_{f}}{\rightleftharpoons}}$ & NO + O & $1.5\times10^{-14} T \exp(-3270/T)$\\
                  \hline
		\end{tabular}
	\end{center}
\end{table}



\begin{figure*}
 	\includegraphics[width=0.48\textwidth]{figs/test_reverse/k1reverse.eps}
 	\includegraphics[width=0.48\textwidth]{figs/test_reverse/k2reverse.eps}
         \caption{Comparison between the rate coefficients obtained with the reverse kinetic module of \kromes, with the experimental and theoretical data from  \citet{Baulch1994}. Left panel: NO+N$\to$N$_2$+O, right panel: NO+O$\to$O$_2$+N. }
 \label{fig:reverse_kr}
\end{figure*}

\begin{figure}
 	\includegraphics[width=0.48\textwidth]{figs/test_reverse/reverse.eps}
         \caption{Time evolution of the species of the Zel'dovich nitric oxide (NO) mechanism.}
 \label{fig:reverse_evol}
\end{figure}


